Investigating Why Contrastive Learning Benefits Robustness Against Label Noise

Self-supervised Contrastive Learning (CL) has been recently shown to be very effective in preventing deep networks from overfitting noisy labels. Despite its empirical success, the theoretical understanding of the effect of contrastive learning on boosting robustness is very limited. In this work, we rigorously prove that the representation matrix learned by contrastive learning boosts robustness, by having: (i) one prominent singular value corresponding to each sub-class in the data, and significantly smaller remaining singular values; and (ii) {a large alignment between the prominent singular vectors and the clean labels of each sub-class. The above properties enable a linear layer trained on such representations to effectively learn the clean labels without overfitting the noise.} We further show that the low-rank structure of the Jacobian of deep networks pre-trained with contrastive learning allows them to achieve a superior performance initially, when fine-tuned on noisy labels. Finally, we demonstrate that the initial robustness provided by contrastive learning enables robust training methods to achieve state-of-the-art performance under extreme noise levels, e.g., an average of 27.18\% and 15.58\% increase in accuracy on CIFAR-10 and CIFAR-100 with 80\% symmetric noisy labels, and 4.11\% increase in accuracy on WebVision.

==> analysis.tex <==

\section{Contrastive Learning and Robustness to Label Noise}
While the recent stream of observations [...] show that self-supervised learning greatly improves the robustness under label noise, the reason is yet to be found. \cite{demystifying} try to given an explanation by considering a binary classification task where a linear model is trained on the embeddings output by self-supervised learning. However, their results are based on the assumption that the embeddings follow a simple Gaussian distribution which is a general assumption and not necessarily related to self-supervised learning. In contrast, we start from the very beginning, the distribution of the augmentations and rigorously show that self-supervised learning extracts the underlying subclass information from the augmentation dataset and this information encoded into the embeddings further benefits the training of a linear head under label noise.

Our starting point is \cite{paper_ssl_contra_loss}, who introduce the notion of augmentation graph and point out that the embeddings produced by contrastive learning can be viewed as a low-rank approximation of the normalized augmentation graph. This helps us build the connection between the data distribution and the performance of the linear classifier, based on which we can further figure out which kind of good property of the embeddings helps defend against label noise and where it comes from.

We first formulate the distribution of data augmentations. We use $P$ to denote the distribution of all natural data (raw inputs without augmentation). For a natural datum $x^*\sim P$, let $A(\cdot|x^*)$ be the distribution of $x^*$'s augmentations, that is, for an augmented datum $x$ , $\mathcal{A}(x|x^*)$ is the probability of generating $x$ from $x^*$. Let $w_{x_ix_j}=\mathbb{E}_{x^*\sim P}[\mathcal{A}(x_i|x^*)\mathcal{A}(x_j|x^*)]$, which can be interpreted as the marginal probability of generating $x_i$ and $x_j$ from a random natural data. We have $K$ classes and $\bar{K}\geq K$ subclasses. Although our labels are only dependent on the classes, the underlying distribution of augmentations are dependent on the subclasses. For example, the class of fruit may contain images of apples and oranges, which are the two subclasses. And two augmented orange images look very likely to be generated from some natural image of orange while an augmented apple image and an augmented orange image are barely possible to be generated from the same datum, that is, $w_{\text{orange, another orange}}$ is significantly larger than $w_{\text{orange, apple}}$ with the latter almost zero. 

To formalize the above idea that the augmentation of a datum from one subclass looks very different from one drawn from another subclass and similar enough to one drawn from the same subclass, we make the following two assumptions:
\begin{assumption}\label{assump: block} $w_{x_ix_j} = 0$ if $x_i$ and $x_j$ are from different subclasses.
\end{assumption}

\begin{assumption}\label{assump: ratio} For any $x_s$ and $x_t$ from the same subclass and any $x_j$, if $x_s$ is similar/dissimilar to $x_j$ in terms of the marginal probability of being generated from a natural datum, then $x_t$ is also similar/dissimilar to $x_j$. Formally,
\begin{align}
    \nonumber
    \frac{w_{x_s x_j}}{w_{x_t x_j}} \leq 1+\delta',
\end{align}
here we take $0/0=1$.
\end{assumption}

We can relax assumption \ref{assump: block} to a more general case where $w_{x_ix_j}$ with $x_i$ and $x_j$ from different subclasses can be very small but non-zero. See Appendix. 

We consider the following loss \cite{paper_ssl_contra_loss} for contrastive learning:
\begin{align}
    \nonumber
    \mathfrak{C}(f) = -2\mathbb{E}_{x,x^+}[f(x)^{\top}, f(x^+)]+\mathbb{E}_{x,x^-}[(f(x^{\top})f(x^-))^2],
\end{align}
where $f(x)$ is the output of the encoder network given an input $x$, $x,x^+$ are drawn from the augmentations of the same natural datum and $x,x^-$ are simply to augmentations generated independently (they can be either generated from a common datum or two different data). As is pointed out in \cite{paper_ssl_contra_loss}, this loss is not exactly the same but very close to many popular contrastive losses [...] (and they also give an example that the loss of SimCLR can be written in a very similar form). Therefore our analysis based on this loss still provides useful insights to understand other contrastive learning method with differenct losses.  

After contrastive learning is finished, a linear model is trained on the embeddings output by the encoder. Supposing the size of augmented dataset is $n$ and each augmented datum is labeled by the label of the natural datum it is generated from. Given the one-hot label matrix $Y\in \mathbb{R}^{n\times K}$, the feature matrix $F\in \mathbb{R}^{n\times p}$ where each row is $f(x)^{\top}$ the embedding of a datum, we consider the downstream task as minimizing the squared loss with a linear model parameterized by $W\in \mathbb{R}^{p\times K}$
\begin{equation}
\nonumber
    \min_{W\in \mathbb{R}^{p\times K}} \mathcal{L}(W,F,Y) \coloneqq \frac{1}{2}\|Y-FW\|_F^2.
\end{equation}
We use gradient descent to solve this problem and denote the parameter at the $t$-th iteration by $W_t^{F, Y}$,
\begin{align}
    \nonumber
    W_t^{F, Y} = W_{t-1}^{F, Y} - \eta \nabla_{W}\mathcal{L}(W_{t-1}^{F, Y}, F, Y)
\end{align}
where $\eta$ is the learning rate. For simplicity we assume $W_0^{F, Y}$ is initialized as $0$.

\subsection{Gaussian Label Noise}
Now we consider the case where $Y=\hat{Y}+\Delta Y$ with $\hat{Y}$ the ground-truth label matrix, and $\Delta Y$ the label noise with each column drawn independently from $\mathcal{N} (0, \sigma^2\mathbf{I}_n/K)$. We are interested in the expected training loss w.r.t. the ground-truth label, we call which ground-truth training loss (as opposed to the training loss w.r.t. the noisy labels based on which we do gradient descent), denoted by $\mathbb{E}\mathcal{L}^*$
\begin{align}
    \nonumber
    \mathbb{E}\mathcal{L}^*(t, F) 
    &=
    \mathbb{E}_{\Delta Y} \mathcal{L}(W_t^{F, \hat{Y}+\Delta Y}, F, \hat{Y}) \\
    &= \mathbb{E}_{\Delta Y} \frac{1}{2}\|\hat{Y}-FW_t^{F, \hat{Y}+\Delta Y}\|_F^2.
\end{align}
Let $n$ denote the total number of augmentations and $n_{\bar{k}}$ denote the number of augmentations in subclass $\bar{k} \in [\bar{K}]$. The following theorem bounds the ground-truth training loss achieved by the linear model trained on the embeddings output by the minimizer of the contrastive loss.


\begin{theorem}\label{theorem: gaussian_loss}
Let $\hat{F} = [\hat{f}(x_1), \hat{f}(x_2), \dots, \hat{f}(x_n)]^{\top}$, where $ \hat{f} = \argmin_f \mathfrak{C}(f)$ obtained by contrastive learning. Then with assumption \ref{assump: block} and \ref{assump: ratio} hold, let $\delta = (1+\delta')^{3/2}-1$ and we have
\begin{align}
    \label{eq: upper_bound_error}
    \mathbb{E}\mathcal{L}^*(t, \hat{F}) \leq& \underbrace{\frac{1}{2}\left(n-(1-(1-\eta)^{2t})\sum_{\bar{k}=1}^{\bar{K}}  \pi_{\bar{k}}(\delta)n_{\bar{k}}\right)}_{\text{bias}} \\
    &+ \underbrace{\frac{\sigma^2}{2}V_1(\eta, t)+ \frac{\sigma^2}{2}V_2(\eta, t)}_{\text{variance}},
\end{align}
where
% \begin{equation*}
\begin{align}
    &\begin{cases}
      V_1(\eta, t) = \bar{K}(1-(1-\eta)^t)^2, \\
      V_2(\eta, t) = \min\{(t\eta)^2\sum_{\bar{k}=1}^{\bar{K}} \rho_{\bar{k}}(\delta), \quad p-\bar{K}\},
    \end{cases}\\
% \end{align}
% \text{and}%\qquad
% \begin{aligned}[c]
    &\begin{cases}
      \pi_{\bar{k}}(\delta) =  \frac{n_{\bar{k}}}{1+(n_{\bar{k}}-1)(1+\delta)^2}, \\
      \rho_{\bar{k}}(\delta) =  \frac{(1+(n_{\bar{k}}-1)(1+\delta)^2)(1+\delta)^2}{n_{\bar{k}}}-1.
    \end{cases}
\end{align}
% \end{equation*}
\end{theorem}
\begin{remark} We call the first term in the right hand side of equation \ref{eq: upper_bound_error} the bias term, which is the error of the model trained with ground-truth label and decreases during the training. We call the second term the variance term because it results from the label noise and increases during the training. The variance consists of two terms $V_1$ and $V_2$. $V_1 \rightarrow \bar{K}$ as $t\rightarrow \infty$. If $\bar{K}=K$, then $V_1$ can be interpreted as the smallest rank of $F$ required for the linear classifier to distinguish between the $K$ classes. And $V_2$ is the error caused by other unnecessary components in $F$, the speed at which it grows is dependent on $\delta$. A small $\delta$, which means a compact subclass structure in terms of the augmentation distribution, makes $V_2$ increases slowly during the training, leaving enough time for the bias to get essentially small before the variance become too large. And in the best case where $\delta=0$, since $\pi_{\bar{k}}(\delta)=1$ and $\rho_{\bar{k}}(\delta)=0$, the bias term tends to $0$ with $V_2$ remaining $0$ during the training. This theorem suggests that contrastive learning exploits the underlying subclass structure in the augmentations to help defend against the noise. As a result a low error w.r.t. the ground-truth labels is guaranteed despite that the linear classifier is trained with corrupted labels. 
\end{remark}

\subsection{Label Flipping}
Next we study the case where $\Delta Y$ is generated by label flipping, which is actually what happens in real-world scenarios. For each data $x_i$, if $x_i$ is from class $j$ with its label flipped to class $k$, then $\Delta Y_{i, j} = -1$ and $\Delta Y_{i, k} = 1$ with other entries in the $i$-th row being $0$; if the label of $x_i$ is not corrupted then all the entries in the $i$-th row of $\Delta Y$ are $0$. Our next theorem shows that there is even some case where the linear classifier trained on $\hat{F}$ can recover all the labels in the training set under label flipping. Let $\alpha_{\bar{k}}$ be the fraction of corrupted data in subclass $\bar{k}$. For simplicity we assume that the $\alpha_{\bar{k}} n_{\bar{k}}$ corrupted data in subclass $\bar{k}$ have their labels evenly flipped to the other $K-1$ classes, i.e., $\alpha_{\bar{k}} n_{\bar{k}}/(K-1)$ for each, despite that our result can be trivially extended to more unbalanced cases.
\begin{theorem}\label{theorem: flipping_accuracy}
Let $n_{\min} = \min\{n_1, \dots, n_{\bar{K}}\}$, $n_{\max} = \max\{n_1, \dots, n_{\bar{K}}\}$, $\bar{k}_{\max} = \argmax_{\bar{k}\in[\bar{K}]}n_{\bar{k}}$ and $\alpha_{\max} = \max\{\alpha_1, \dots, \alpha_{\bar{K}} \}$. The accuracy w.r.t. the ground-truth labels of the training data is defined as 
\begin{align}
    \nonumber
    &Accuracy^*(t,F,\Delta Y) =\\ &~~~~\frac{1}{n} \sum_{i=1}^n \mathbbm{1}\left[\argmax_{j\in[K]} (FW_t^{F, \hat{Y}+\Delta Y})_{i,j} = \arg_{j\in [K]}(\hat{Y}_{i,j}=1) \right]
\end{align}
Given $\epsilon_1, \epsilon_2\in(0,1)$, the linear classifier trained on $\hat{F}$ can achieve a 100\% ground-truth accuracy, i.e., $Accuracy^*(t, \hat{F}, \Delta Y) = 1$ when
\begin{align}
    \nonumber
    &t\in [\frac{\ln\frac{1}{\epsilon_2}}{\ln \frac{1}{1-\eta}}, \frac{\epsilon_1}{\Psi(\eta, \delta)}], \\%\quad \text{and}\quad 
    &\alpha_{\max} < \frac{(1-\frac{1}{\pi_{\bar{k}_{\max}}(\delta)}\frac{2\epsilon_1}{1-\epsilon_2}\frac{n_{\max}}{n_{\min}})(K-1)}{K-1+\frac{n_{\max}}{n_{\min}}\Omega(\delta)},
\end{align}
where
\begin{align}
&\Psi(\eta, \delta) = \eta \sqrt{(p-\bar{K}+1)n_{\max}\rho_{\bar{k}_{\max}}(\delta)},\\%\quad 
&\Omega(\delta) = \frac{(1+\delta)^2(1+(1+\delta)^2(n_{\max}-1))}{n_{\max}-1+(1+\delta)^2}.
\end{align}
\end{theorem}

\yx{An equivalent statement; feel like the following one is better}
\begin{theorem}\label{theorem: flipping_accuracy}
Let $n_{\min} = \min\{n_1, \dots, n_{\bar{K}}\}$, $n_{\max} = \max\{n_1, \dots, n_{\bar{K}}\}$, $\bar{k}_{\max} = \argmax_{\bar{k}\in[\bar{K}]}n_{\bar{k}}$ and $\alpha_{\max} = \max\{\alpha_1, \dots, \alpha_{\bar{K}} \}$. The accuracy w.r.t. the ground-truth labels of the training data is defined as 
\begin{align}
    \nonumber
    &Accuracy^*(t,F,\Delta Y) =\\ &~~~~\frac{1}{n} \sum_{i=1}^n \mathbbm{1}\left[\argmax_{j\in[K]} (FW_t^{F, \hat{Y}+\Delta Y})_{i,j} = \arg_{j\in [K]}(\hat{Y}_{i,j}=1) \right]
\end{align}
Given $\epsilon_1\in[0, 1), \epsilon_2\in(0,1)$, if $\delta \leq \Psi(\epsilon_1, \epsilon_2)$, then as long as 
\begin{align}
    \label{eq: tolerance}
    \alpha_{\max} < \frac{(1-\frac{1}{\pi_{\bar{k}_{\max}}(\delta)}\frac{2\epsilon_1}{1-\epsilon_2}\frac{n_{\max}}{n_{\min}})(K-1)}{K-1+\frac{n_{\max}}{n_{\min}}\Omega(\delta)},
\end{align}
there exists an interval $[t_1, t_2]$ s.t. when trained on $\hat{F}$ for $t\in [t_1, t_2]$ iterations the linear classifier achieves a 100\% ground-truth accuracy, i.e. $Accuracy^*(t, \hat{F}, \Delta Y) = 1$. 

 $\pi_{\bar{k}_{\max}}(\delta)$ is as defined in theorem \ref{theorem: gaussian_loss} and $\Psi(\epsilon_1, \epsilon_2, n_{\max})$ and $\Omega(\delta)$ are defined as follows
\begin{align}
    \nonumber
    \Psi(\epsilon_1, \epsilon_2) = & \sqrt{\frac{\sqrt{4(n_{\max}-1)(\psi(\epsilon_1, \epsilon_2)+1)n_{\max}}-1}{2(n_{\max}-1)}}-1, \\
    \nonumber
    \Omega(\delta) = & \frac{(1+\delta)^2(1+(1+\delta)^2(n_{\max}-1))}{n_{\max}-1+(1+\delta)^2}.
\end{align}
where 
\begin{align}
    \nonumber
    \psi(\epsilon_1, \epsilon_2) = \left(\frac{\ln\left(1-\frac{\epsilon_1}{\sqrt{n_{\max}}(p-\bar{K}+1)}\right)}{\ln\epsilon_2}\right)^2.
\end{align}
It is easy to check that $\Psi(\epsilon_1, \epsilon_2, n_{\max})$ is always $\geq 0$.
\end{theorem}

\begin{remark}
Theorem \ref{theorem: flipping_accuracy} shows the exact conditions under which the linear classifier can recover all the corrupted labels. The noise tolerance given in equation \ref{eq: tolerance} is dependent on some properties of the dataset ($n_{\max}$, $n_{\min}$, K) as well as $\epsilon_1$ and $\epsilon_1$ that one can set. Smaller $\epsilon_1$ and $\epsilon_1$ lead to a higher tolerance but requires a smaller $\delta$, i.e., a more structured augmentation dataset. Alternatively speaking, a smaller $\delta$ allows one to choose smaller $\epsilon_1$ and $\epsilon_2$ to satisfy $\delta \leq \Psi(\epsilon_1, \epsilon_2)$, which implies a higher noise tolerance. Note that $\Omega(0)=1$ and $\pi_{\bar{k}}(0)=1$ means in the best case where $\delta=0$, $\epsilon_1$ can be as small as $0$, supposing $n_{\max}=n_{\min}$, the tolerance will be exactly $(K-1)/K$.
\end{remark}
